A Parallel SystemC Virtual Platform for Neuromorphic Architectures

With the increasing interest in neuromorphic computing, designers of embedded systems face the challenge of efficiently simulating such platforms to enable architecture design exploration early in the development cycle. Executing artificial neural network applications on neuromorphic systems which are being simulated on virtual platforms (VPs) is an extremely demanding computational task. Nevertheless, it is a vital benchmarking task for comparing different possible architectures. Therefore, exploiting the multicore capabilities of the VP's host system is essential to achieve faster simulations. Hence, this paper presents a parallel SystemC based VP for RISC-V multicore platforms integrating multiple computing-in-memory neuromorphic accelerators. In this paper, different VP segmentation architectures are explored for the integration of neuromorphic accelerators and are shown their corresponding speedup simulations compared to conventional sequential SystemC execution.

==> rw.tex <==
Electronic system level (ESL) parallel discrete event simulation is a field well researched in academia. However, such parallelization still has not yet found its way into mainstream ESL simulation. VPs commonly use SystemC as their underlying simulation engine, which deploys a standard discrete event approach to simulate the concurrency of multiprocessor systems. There are several approaches for parallelization of SystemC \cite{ParalleSysC1,OoOparallelsym,LegaSCI}. A synchronous approach to parallel SystemC simulation is presented in \cite{LegaSCI}. Synchronous techniques, however, are unable to exploit the full parallelism of a simulation, given that they enforce strict time synchronization among all threads. This synchronous limitation can be overcome by applying a time-decoupled technique as proposed in \cite{timedecoup}. These techniques have been applied in \cite{SysCArm} to multicore VPs for specific workloads like booting operating systems and for network intensive communication applications. However for heavy VMM operations needed in machine learning applications, that are executed in a system-level VP with multiple neuromorphic accelerators architecture, there is limited work available. Extensive work on different simulators for neuromorphic architectures with different abstraction levels is summarized in~\cite{neurosurvey2}, where the majority of simulators focus on circuit level. Only a few works like~\cite{ICESOCC,TechnionSystemL} have presented complete integration of neuromorphic accelerators into a full system. However, they have not been explicitly developed to exploit the multicore nature of their host systems. Therefore, this work presents a time-decoupled parallel simulation framework that allows different VP segmentation strategies of neuromorphic architectures.
